A Multi-scale Visual Analytics Approach for Exploring Biomedical Knowledge

This paper describes an ongoing multi-scale visual analytics approach for exploring and analyzing biomedical knowledge at scale.We utilize global and local views, hierarchical and flow-based graph layouts, multi-faceted search, neighborhood recommendations, and document visualizations to help researchers interactively explore, query, and analyze biological graphs against the backdrop of biomedical knowledge. The generality of our approach - insofar as it re-quires only knowledge graphs linked to documents - means it can support a range of therapeutic use cases across different domains, from disease propagation to drug discovery. Early interactions with domain experts support our approach for use cases with graphs with over 40,000 nodes and 350,000 edges.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Workshop VIS 2021 - Short paper/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Workshop VIS 2021 - Short paper/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> Workshop VIS 2021 - Short paper/sections/1-introduction.tex <==
\section{Introduction}
With over 1.5 million publications a year and more than 50 million peer-reviewed articles in existence, the rate and volume of novel scientific research remains overwhelming, having long surpassed our ability to fully understand and utilize what is known \cite{jinha2010article}. Crises like the COVID-19 pandemic only exacerbate this situation, with critical information dispersed across the papers published each day \cite{hechenbleikner_data_2020}. To stay up-to-date, scientists must manually review publications to internalize new knowledge. Therefore, their coverage of the field remains small, and at this scale and pace, contextualization of new knowledge and synthesis with prior knowledge is often impractical, biased, and error-prone. 
% When time pressures meets information overload, science is forced into ``crisis-response'' mode \cite{Lee:_2021}, with workflows that take years being compressed into months. 
While all disciplines are subject to the effects of rapidly-changing knowledge, the cost in medical research can be measured in human lives.
 
In the field of biomedicine, it is already difficult and time-consuming to develop and validate hypotheses. Against the backdrop of all scientific knowledge, biomedical researchers start with a certain question, and turn to their prior domain knowledge and the mental models from their specific experiences \cite{janes_engineering_2017}. As many biological processes are inherently network phenomena, they are well suited for graph analysis \cite{sosa_literature-based_2019}. For example, when analyzing the effects of a drug on a disease, biomedical researchers must assemble (or update) biological graphs from literature, analyze their causal structure, extract relevant subgraphs, highlight novel or alternative pathways that could aid in drug discovery, flag potential viral mutations should new pathways appear, and distill all this analysis into a list of drug candidates for downstream trials. Similar graph analytic workflows are required across a range of biomedical use cases. However, the sheer size and dense connectivity of such graphs makes them hard to visualize and analyze in real-time. 
% Existing tools and approaches\cite{INDRA_pathwaymap, SIGNOR, DialogueBio} help researchers to test and validate pathways and subgraph structures. A number of challenges remain, however. The sheer size and dense connectivity of these graphs makes them hard to visualize and interact with in real-time. 
% Moreover, since such workflows require starting from prior knowledge, they tend to have a biasing effect towards local graph exploration, particularly without context-informed, system-guided exploration of these graphs and relevant literature.

The primary research contribution of this paper is a multi-scale visual analytics approach that enables the investigation of biological graphs to facilitate a variety of use cases such as drug discovery, disease analysis, and identification of side-effects. This research is part of our ongoing effort for DARPA's Automating Scientific Knowledge (ASKE) program \cite{ASKE}.
% It leverages global and local views, hierarchical and flow-based graph layouts, multi-faceted search, system recommendations, and document visualization approaches to help biomedical researchers interactively explore, query, analyze, and expand automatically-extracted, literature-derived \rv{biological} models. 
Utilizing data from our ASKE collaborators \cite{INDRA, cosmos}, we developed a web-based prototype that visualizes 16 biological graphs against a corpus of 176,000 documents. 
We then conducted an expert evaluation in order to better understand how the system helps biomedical researchers in identifying drug-target interactions. 
Domain experts believe our approach to have unique value for knowledge exploration, and our initial iteration with users underscored that the prototype was easy to interact with and useful for navigating and analyzing large graphs against the backdrop of scientific knowledge. More generally, we believe our design approach is flexible enough to be used for knowledge discovery in other graph-based domains. 

% We also identify and describe several use cases for the prototype to demonstrate its clinical significance... % describe the features used in the system
% We then evaluated the efficacy of the system in a user study in which biologists worked to conduct biological queries and look for the underlying knowledge. 


==> Workshop VIS 2021 - Short paper/sections/2-relatedwork.tex <==
\section{Related Work}
% This section describes other relevant prior works that have proposed visualization solutions for biological graphs and large-scale scientific knowledge exploration. 

\subsection{Biological Graph Visualization}
Graph-based visualizations remain key to understanding biological graphs across a range of use cases \cite{gehlenborg_visualization_2010, pavlopoulos_survey_2008}. Most existing visualization approaches support static overviews of the entire graph \cite{kanehisa_kegg_2000, jeske_brenda_2019} and interactive views of focused subgraphs \cite{INDRA_pathwaymap, DialogueBio, SIGNOR}.
However, research has shown that the inherent multi-scale nature of biological graphs can only be fully appreciated when the entire range from local to global graph structures can be inspected continuously and interactively \cite{pirch_vrnetzer_2021}. 
% Moreover, a previous survey on biological graph visualization discovered that the majority of tools can cope with datasets of up to about 5,000 nodes without severely compromising speed and user friendliness \cite{pavlopoulos_survey_2008} .
Some tools such as Reactome \cite{sidiropoulos_reactome_2017} strike a balance by displaying overviews of biological graphs as well as detailed views of selected subgraphs or pathways. Yet, in the workflow, the overviews are replaced by selected pathways and thus global insight is decreased. By contrast, we propose a novel approach for scalable and performant graph analysis with coordinated and adjustable global and local views so the multi-scale character of biological graphs can be preserved and interrogated with multi-faceted search, interactive navigation, and progressive drill-down on demand.
% We also focus on automatically-extracted, literature-derived \rv{biological} models, which represent regulation between two or more biological agents.

% However, making sense of large graphs is a fundamental challenge due to the size and the complexity of biological models \cite{wu_graph_2019}, with few tools that allow biologists to explore, visualize, and understand them. \cite{pienta_scalable_2015}.
% Existing biological visualization approaches are categorized into two broad types: static overviews of the entire graph (\texit{global}) or interactive small-scale views of subgraphs (\textit{local}).

% Visualization tools that employ the global approach showing overview maps of metabolic pathways include the \texit{Kyoto Encyclopedia of Genes and Genomes (KEGG)} \cite{kanehisa_kegg_2000} and \textit{BRENDA} \cite{jeske_brenda_2019}, which was drawn using the network editor Cytoscape \cite{shannon_cytoscape_2003}. 
% In contrast, the Small Molecule Pathway Database (SMPDB) \cite{frolkis_smpdb_2010} and \textit{WikiPathways} \cite{slenter_wikipathways_2018} provide visualizations of small scale human metabolic pathways and biological pathways respectively, which were not integrated into an overview map.
% Similarly, systems like Entourage \cite{lex_entourage_2013} and enRoute \cite{partl_enroute_2013} visualize relationships between biological pathways but focus on one pathway map while displaying contextual pathways or associated experimental data. 
% Unlike other tools, \textit{Reactome} first provides a hierarchical visualization to show relationships between biological pathway categories, which later zooms into a subgraph with detailed information after the user selects a particular category \cite{sidiropoulos_reactome_2017}. 
% New visualizations have also been proposed such as \textit{Metabopolis} \cite{wu_metabopolis_2019} which uses an urban map to create a visual hierarchy of biological pathways.

% Research has shown that the inherent multi-scale nature of biological processes can only be fully appreciated when the entire range from local to global network structures can be inspected continuously and interactively \cite{pirch_vrnetzer_2021}.
% To address the limitations of presenting either static overviews or small subgraph views, we propose an approach for graph analysis that combines both by displaying two coordinated global and local views. 

\subsection{Large-Scale Scientific Knowledge Exploration}

% Clustering plays an important role in many large-scale data analyses providing users with an overall understanding of their data \cite{lee_ivisclustering_2012}.
% Document clustering has been investigated for use in a number of different areas of text mining and information retrieval \cite{steinbach_comparison_2000}, including subject headings of library catalogues \cite{miller_nypl_2014}, images from images 19th-century Meserve-Kunhardt Collection \cite{duhaime_visualizing_nodate}, papers in economy \cite{noichl_structure_2019}, papers in philosophy \cite{noichl_modeling_2021}, book or article assigned in the Open Syllabus corpus \cite{mcclure_galaxy_2021}, tweets about coronavirus \cite{kibardin_what_2020}, and articles in the COVID-19 Open Research Challenge \cite{kibardin_using_2020}, and text documents in general \cite{carrot_search_lingo4g_2021}. 

Visualizations of large-scale scientific corpora can be broadly categorized into citation-linked graphs \cite{gates_nature_2019, eitan_connected_2021} and similarity clusters \cite{stasko_jigsaw_2013, kibardin_using_2020}.
%, goulard_mapping_2021, kibardin_using_2020}. 
Citation-linked graphs represent articles as nodes and edges as citations. Cluster visualizations typically apply dimensionality reduction to produce text embeddings that can be visualized as interactive 2-D scatterplots. For example, Open Knowledge Maps \cite{kraker_open_2016} displays clusters of PubMed \cite{PubMed} articles based on textual similarity.
% Clusters are formed automatically with similar articles placed close to each other. 
More recent approaches visualize biomedical data repositories and scientific articles, using metadata for overview, organization, custom user-feeds and semantic querying \cite{lekschas_satori_2018, kraker_open_2016, kerren_biovis_2017}. 
% SATORI\cite{lekschas_satori_2018} is a visual analytics tool that leverages metadata to provide a hierarchical overview of biomedical datasets and enables semantic querying. 
  
% The BioVis Explorer\cite{kerren_biovis_2017} displays articles related to biological visualization in a 2-D map, where edges are displayed on demand connecting articles that utilize similar visualization techniques. BioFactoid \cite{} allows researchers to create their own articles' profiles and connects them with relevant literature.

Taking inspiration from the above work, we are building the capability for interactive exploration of hierarchical clusters of scientific knowledge, where nested sub-clusters organize related knowledge at finer resolution. To our knowledge, this visual and interactive approach is not yet present in the field at large. 

% Our collaborators are also able to connect source knowledge with existing \rv{biological} graphs, which builds trust in these graphs. 


% For example, 38 million articles indexed in Clarivate Analytics’ Web of Science (WoS)  were visualized as a co-citation graph. % where dots representing articles are linked if another paper cites both. The use of color shows different disciplines. 
% Although the network provides a summary overview and differentiates papers cited by different disciplines or deeply embedded in their own discipline, there are no clearly defined clusters.
% In contrast, similarity clusters such as iVisClustering, which uses the InfoVis and VAST papers data set \cite{stasko_jigsaw_2013}, shows a graph-based layout of papers categorized based on their topic \cite{lee_ivisclustering_2012}. 
% %In such visualizations, scientific articles tend to bunch together according to age and topic because authors usually reference recent articles related to their paper’s subject \cite{mukherjee_nearly_2017} and clusters are clearly defined. 
% However, this system was limited in its scalability since only 454 titles and abstracts were used. 

% To visualize biomedical data repositories, SATORI provides a node-link diagram of metadata attributes extracted from the dataset based on their subclass relationships defined by the ontologies \cite{lekschas_satori_2018}. The hierarchical structure of ontologies specific to biomedical data allows nodes to be connected by an ‘is superclass of’ relationship. 
% % The node-link technique provides a visual representation of the similarity between related terms and emphasizes the hierarchical structure of the annotation term graph. 

% Knowl provides both a force-directed graph with each node linked by citations and a dimensions reduction map clustered by keywords \cite{goulard_mapping_2021}. Their user evaluation revealed that participants were more comfortable with the keyword cluster graph. 
% We adopt a similar approach as the dimensions reduction map to represent the corpus of biological knowledge to make it easier to understand. 

% Through a review of current approaches, we drew insights to incorporate in our design for the representation of articles in biology. 
% We found that the existing approaches are focused on providing a good overview of the underlying corpus but they have limited interactions such as drill-down and filtering. 
% Additionally, the link back to the original document is not always present, which makes it difficult to trace back to where a piece of information comes from.
% Similarly, the search functionality is not always present or limited, making it difficult to find specific documents. 
% Thus, in our interface, we seek to support better interactions, links to original publications, and querying capabilities. 
%Overuse of color to encode clusters/groups and highlighting, which can be difficult to differentiate when the number of groups/categories gets larger
%Hierarchical layouts are rarely used. Most of the approaches rely on semantic zooming to show more details on demand (top N documents within a cluster, labels, etc.)
%Some of these approaches work with fixed ontologies or categories (e.g. scientific disciplines), which makes easier to provide context
%Overall, there are currently few systems that allow biologists to explore, query, and analyze large scale graphs while providing the underlying contextual information for knowledge discovery. Thus, we propose an integrated system for scalable graph analysis and knowledge discovery. 


==> Workshop VIS 2021 - Short paper/sections/3-designprocess.tex <==
\section{Design Process and Goals}

Our user-centered design process was based on periodic meetings over eight months with domain experts and stakeholders in systems biology, bioinformatics, and causal reasoning applied to the study of infectious diseases. Based on these interactions, we identified the following high-level design goals (DG):
%The following high-level design goals (DG) were identified: 
\begin{itemize}
	\setlength\itemsep{0pt}
    \item \textbf{DG1. Provide scalable, interactive, and performant visualizations of biological graphs.} Such graphs range from small ones visualized in standard ways to those with over tens of thousands of nodes and hundreds of thousands of edges. The visualization approach should therefore be scalable with real-time interactivity, and should organize knowledge to be as visually digestible as possible.   
    Leveraging the data and ontology provided by our knowledge assembly collaborators \cite{EMMAA, INDRA}, our approach should enable biomedical researchers to query and analyze the high-level structures of biological graphs derived from domain literature, thereby gaining insight on the ontological structure of the extracted causal knowledge.
    \item \textbf{DG2. Provide iterative local analysis coordinated with global context.} While interactive graph overviews are useful to identify high-level structural and ontological patterns, biomedical researchers need to isolate and extract relevant subgraphs for more focused analysis. They also need to iterate on these subgraphs as needed while keeping global context in mind. For example, to judge drug side effects, our approach must enable researchers to identify incoming and outgoing pathways from particular agents, and iteratively expand or truncate the subgraph under analysis in light of all pathways available in the global graph. 
    \item \textbf{DG3. Promote scientific knowledge synthesis and discovery.} Researchers should be able to access backing scientific corpora to further contextualize their analysis and explore related knowledge spaces. Using data provided by our collaborators \cite{EMMAA, INDRA, cosmos}, our visualization approach allow researchers to seamlessly navigate back and forth from biological graphs to the scientific corpus at large. In this manner, researchers can trace pathways expressed in graph form to source documents and explore related knowledge to broaden their analysis. 
\end{itemize} 

==> Workshop VIS 2021 - Short paper/sections/4-data-preprocessing.tex <==
\section{Data Processing}
Our approach leverages graph and knowledge data from collaborating systems in INDRA and COSMOS. INDRA (the Integrated Network and Dynamical Reasoning Assembler) assembles a network of biological processes from statements extracted from source documents using natural language processing techniques \cite{INDRA}. Extracted mechanistic and causal assertions are standardized and mapped to a biological ontology \cite{INDRA_BioOntology}, generating an assembled set of causal statements that constitute a biological graph . We further normalize this statement data into a multidigraph optimized for real-time browser rendering. Here, biological agents are mapped to nodes clustered as per their ontological category and causal statements are mapped to directed edges between agents, with edges bundled into hyper-edges to enable layout generation at each level of the ontology. 

COSMOS is a knowledge discovery platform that automates the process of extracting and assimilating heterogeneous artifacts from diverse scientific publications \cite{cosmos}. In addition to enabling search over a large corpus of publications, COSMOS extracts tables, text, images and source code. The corpus provided by COSMOS consists of 176,000 documents, complete with metadata and document artifact extraction. Knowledge search over this corpus is made available in our prototype via API. The corpus is also available as an embedding dataset, with each document cast as a vector embedding \cite{rehurek_lrec}. To these embeddings, we apply dimensional reduction via UMAP and hierarchical clustering via HDBSCAN to first project the embeddings into a 2D space and then group semantically proximate documents as nested clusters \cite{McInnes2017, mcinnes_umap_2020}. Moreover, for each cluster, we compute the alpha shape of its point subspace to establish a polygon cluster boundary \cite{edelsbrunner_shape_1983}.

% These representations or embeddings are then projected down to two dimensions using the dimension reduction technique known as UMAP 
% and presented as a two-dimensional distribution of dots. Each dot is a document and the distance between each pair of dots measures the syntactic similarity of the underlying text.
%The resulting points are presented as a topological 2-D map with each dot on the map representing an article, where similar articles are placed close to each other. 






==> Workshop VIS 2021 - Short paper/sections/5-system-interface.tex <==
\section{Visualization Design}
The following two subsections describe the two main spaces of our approach - the Graphs space and the Knowledge space - that were developed in light of the above design goals (DG). While the skeleton and core components of our approach are in place, we continue to refine the visualization, interaction, and analytic design for both spaces with domain experts.  

\subsection{Graphs Space}
The Graphs space is composed of two coordinated views (Fig. \ref{fig:teaser}) that seek to simultaneously provide the global and local perspectives needed for multi-scale graph sense-making \cite{pienta_scalable_2015}. As the default view, the \textit{Global View} (Fig. \ref{fig:teaser}. A) provides a visual overview of a biological graph, and has multi-faceted search, real-time navigation, and semantic zoom. The \textit{Local View} (Fig. \ref{fig:teaser}. B) is a sandbox to which search results can be iteratively added as a flow graph for further inspection. Our coordinated approach uses linked filtering and highlighting so changes in one view are reflected in the other. In this way, we look to enable biomedical researchers to engage in local subgraph analysis while contextualizing this analysis within the global context of the large-scale graph. 

\subsubsection{Global View}
The Global View shows an overview of a selected biological graph [\textbf{DG1}] assembled from large sets of biological causal statements. Each causal statement represents regulations between biological agents such as proteins or viruses (e.g. CDC12 phosporylates MID1). The overview global graph displays nested clusters of biological agents organized in the background biomedical ontology. 
% This overview allows biomedical researchers to analyze the high-level graph structure. 
% These causal statements are aggregated at the biological concept level (e.g. molecular entity). 
% Causal statements such as the ones representing complexes not always map one-to-one to model edges since they sometimes have more than one biological agent. We address this by drawing undirected edges between the agents involved in a complex.
We use a hierarchical circle-packing graph layout\cite{d3-hierarchy_2021} to show high-level relationship structure and the nested concepts of the ontology [\textbf{DG1}]. Each ontological group is rendered as rings (in blue) around their children (in orange). To avoid displaying hundreds of thousands of edges, we also apply edge bundling techniques\cite{holten_hierarchical_2006}, where edges with multiple nodes grounded to the same ontological category are bundled into hyper-edges. Hyper-edges are also wrapped around ontological rings to avoid edge clutter between groups, and hyper-edge brightness corresponds to the number of bundled statements. Semantic zooming progressively discloses the nested categories of the ontology as the researcher dives deeper into an ontological branch. 
% In this way, the global view helps researchers to identify high-level patterns of relationships at-a-glance.

This view also allows researchers to interrogate biological graphs by using multi-faceted queries [\textbf{DG2}]. Researchers can chain multiple queries related to node attributes (e.g. node degree), edge attributes (e.g. edge type), and path queries via a search box at the top of the Graphs space (Fig. \ref{fig:teaser}). Query results are displayed on the Global View using contrast-based highlighting, with results foregrounded and the rest of the graph faded out.

\subsubsection{Local View}
While such global views provide high-level structural information, they face sense-making challenges for multi-scale graphs\cite{keim_visual_2001, holten_hierarchical_2006, pienta_scalable_2015}. To this end, we coordinate the Global View with the Local View (Fig. \ref{fig:teaser}.B), where the latter displays a subgraph containing the subset of causal statements resulting from preceding search queries [\textbf{DG2}]. 

Edges are visually encoded based on the implied polarity of the regulation type (e.g. activation, inhibition), curation state (human-verified or unexamined), and directionality (directed or not). We use the following scale to encode edge polarity: blue for ``positive'', red for ``negative'', and gray for ``unknown.'' We use a filled arrow for directed edges and a filled box arrow for undirected edges. Human-verified statements are shown with a filled circle, and unexamined statements have empty circles (incorrect statements are removed during data pre-processing) (Fig. \ref{fig:teaser}. B). As directionality is critical for understanding causality \cite{Wright:2018}, we use a traditional left-to-right flow layout algorithm\cite{Sugiyama:1981} with recent extensions \cite{elkjs:2020}. 
% The layout is also adaptive based on the size of the graph,
% with slightly reduced spacing constraints for larger graphs to offset the
% number of ``lanes'' created by the layout algorithm.

Selecting a node in the Local View opens a Drill-down Panel for the Graphs Space to show node metadata (e.g. agent description) and link suggestions for incoming and outgoing relationships ranked by supporting evidence [\textbf{DG2}]. Neighborhood suggestions are also highlighted in the Global View so researchers can visualize the global connectivity of a given node. Selecting one or more of these relationship suggestions adds them to the subgraph, which helps with neighborhood expansion. 

\subsubsection{Graphs to Knowledge}
To aid trust-building, researchers need to link their graph exploration back to scientific knowledge [\textbf{DG3}]. We build on the links present in the provided data. For example, selecting an edge reveals the underlying evidence extracted by INDRA, where this evidence is surfaced as a short-text fragment (Fig. \ref{fig:teaser}. C). Clicking the text opens a modal dialog displaying associated metadata on both source and neighborhood documents provided by COSMOS. The neighborhood of a given document is taken as the set of semantically similar documents within the corpus\cite{rehurek_lrec}. In this manner, researchers can seamlessly trace a graph edge to its underlying textual evidence and then to the backing scientific paper.


% This metadata is fetched COSMOS, an existing open-source large-scale knowledge discovery platform via APIs that leverages document vector embeddings to find related documents\cite{cosmos}. By following the link at the bottom, it is also possible to visualize the source document in the context of the full corpus of documents in the Knowledge view.

% This metadata is fetched from COSMOS\cite{cosmos}, an existing open-source large-scale knowledge discovery platform that provides API endpoints to machine-generated annotations of 
% scientific publications\cite{goswami_2019}. The neighborhood of a given document is therein defined as the set of the ten most syntactically similar documents within the corpus, 
% as measured by the cosine similarity between their Doc2Vec embeddings\cite{rehurek_lrec}.



% The \textit{overview/detail strategy} employed by the prototype allows subgraphs to be collapsed or expanded upon demand, which can overcome the challenges that face a single view and yield improvements in understanding data \cite{van_den_elzen_multivariate_2014} and more effectively exploring large graphs \cite{odonoghue_visualization_2018}.
 

% We propose an approach for scalable graph analysis wherein two coordinated views enable biologists to interactively explore, query, and analyze graphs at different scales. 
% While the \textit{global} view give a high-level overview of the data by drawing the whole graph dataset \cite{pienta_scalable_2015}, which works well for many domains but face challenges when applied to million-scale graphs \cite{keim_visual_2001, holten_hierarchical_2006}. 
% In contrast, \textit{local} view show only a subset of the entire graph data, which may improve visual comprehension but decrease global insight \cite{pienta_scalable_2015}.
% The \textit{overview/detail strategy} employed by the prototype allows subgraphs to be collapsed or expanded upon demand, which can overcome the challenges that face a single view and yield improvements in understanding data \cite{van_den_elzen_multivariate_2014} and more effectively exploring large graphs \cite{odonoghue_visualization_2018}.

% To visualize large graphs, we needed to structure the data in the \textit{global} view. We started by hierarchically clustering the data based on their biomedical ontology. 
% Each cluster was rendered as rings around their children using a circle packing layout. 
% Due to the large quantity of edges connecting the nodes, the overview graph resembled a ``hairball''. To combat this issue, edges within the same cluster were bundled before exiting the cluster they belong to and edges were curved to smooth out the transition.
% Bundling edges between clusters makes connections visible from a zoomed out view, but continues to generate too much noise when zoomed in. 
% To address this, we further tailored the edges to curve around clusters that do not contain their source or target nodes to make it easier to follow them. In this way, the \textit{global} view shows a hierarchical network with hyper-edges bundled according to zoom level. 

% To explore the large graph in the global view, real-time graph queries are provided, which produce results as highlighted graph sections with blinking nodes. 
% These queries range from simple keyword searches for a node or ontology category and filters for nodes and links with specified attributes, to complex path-finding searches between two nodes. 
% A combination of multiple queries are also supported to generate more specific results. 

% The query results can be extracted as subgraphs into a \textit{local} view, which provides a flow-layout that allows the user to further examine the network of interest. 
% Local subgraphs can be interactively expanded via machine-assisted suggestions, and specific graph elements can be interrogated for source knowledge from scientific literature. 


\subsection{Knowledge Space} 
% \begin{figure}[tb]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/cluster_view.png}
%  \caption{The Clusters View represents the document corpus as an interactive 2D topology, where cluster members (documents) have the same colour and are enclosed in a bounding polygon.}
%  \label{fig:knowledge}
% \end{figure}

% \begin{figure}[tb]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/card_view.png}
%  \caption{The Clusters View represents the document corpus as an interactive topological 2-D map, where members of each cluster(documents) are represented as dots and colored the same and enclosed within a bounding alpha shape.}
%  \label{fig:knowledge}
% \end{figure}


The Knowledge space displays an interactive overview of the scientific corpus. The corpus data contains all source material from which all biological graphs have been assembled, thus encouraging moving back and forth between graph-centric analysis and the literature at large [\textbf{DG3}]. Two perspectives on the knowledge corpus [\textbf{DG3}] are available via: a \textit{Card-based View} and a \textit{Clusters View}.

% The document corpus used in this work is ''xDD-COVID-19``, a 176,000-document subset of the COSMOS\cite{cosmos} corpus that contains relevant terms such as ''SARS-CoV-2``, ''COVID-19``, ''betacoronavirus``, and ''2019nCoV``.
%% Footnote(?): A complete list of the target terms can be found at https://xdd.wisc.edu/api/dictionaries?dictionary=covid-19&show_terms=true
%%To ingest these corpus of documents, we again leverage COSMOS APIs\cite{cosmos}. 
% The goal of the Knowledge space is to enable biomedical researchers to explore large-scale scientific knowledge for context and discovery of related content .

\subsubsection{Card-based View}
The Card-based View has a tabular layout with each document as a card, including a preview image of a document artifact and title. Cards organize information in chunks, which aids in user scannability. As in the Graphs space, the Knowledge space also has rich search capabilities where researchers can perform multiple compound queries on document attributes, including free text, author, publisher, and the presence of artifacts such as tables or figures. 

\subsubsection{Clusters View}

% The Subgraph Embedding has the
% strengths of a scatterplot (including concave hulls around clusters) of
% all the results based on their nodes’ features. The Subgraph Embedding
% allows zooming, panning, jitter, and fine-grain control over embedding
% and clustering. We group similar results with concave hulls, because
% there are many cases in which convex hulls overlap unnecessarily. New
% clusters can be freely created using a freeform lasso tool. Similar
% results are plotted close to each other and often form clusters as in [45].
% The details of our graph embedding algorithm are discussed further in
% Section 4

While the Card-based View supports visual scannability, it suffers from visual scalability for large numbers of documents. The Clusters View (Fig. \ref{fig:knowledge}) thus provides a more scalable perspective on the scientific corpus using document embeddings. Organized in a 2D topology, a point in this visual space is a document, and spatial distance between points measures semantic similarity. Cluster members have the same color and are enclosed within a bounding alpha shape. Documents designated as ``noise'' by the clustering algorithm (not in any cluster) are coloured grey with no boundary. To visually encode cluster hierarchy, color hue is preserved across levels with lower opacity being applied to coarsest clustering levels. 
% This overview allows researchers to build a mental model of the entire corpus and understand the from the cluster labels and their spatial distribution.


% The interface consists of a hierarchical graph with x levels of clusters... 
% describe each level encoding and what nodes represent and how to navigate through the different levels 
% This design addresses the limitations of the flat clustering used in existing visualizations, allowing for progressive disclosure of document clusters as the researcher traverses down the hierarchy. 

% This Clusters View also supports user interactions including zooming and panning. 
% % describe other interactions like hover or click if implemented
% Clicking on a dot also surfaces a citation network where dots are connected when an article cites this particular article. 

% Researchers can also search the space using a multi-faceted search bar at the top which can also be chained and related to keywords, article artifact type, and base and post-processing confidence. 
% The search results are highlighted in the cluster visualization. 

\subsubsection{Metadata and Knowledge to Graphs}
Selecting a document from either a card in the Card-based View or a point in the Clusters View opens a Drill-down Panel in the Knowledge Space with three tabs for deeper interrogation of the document content. The \textit{Preview} tab shows document metadata including title, DOI, authors and publisher-related information, with further drill-down available via a dialog with more detailed information including figures and text excerpts as well as the link back to the source document. This allows the researcher to discover related documents in addition to using spatially proximate documents in the Cluster view. The \textit{Graphs} tab contains links to existing biological graphs in the Graphs space, and fortifies the connection between user analysis and background scientific literature. The \textit{Entities} tab shows related keywords that helps researchers guide subsequent search. 

==> Workshop VIS 2021 - Short paper/sections/6-scenarios.tex <==
\section{Usage Scenario} \label{sec:scenario}

While our approach remains general across various biomedical graph-based use cases, we focus here on a usage scenario relevant to our current era around the exploration of biological mechanisms of COVID-19. A biomedical researcher is investigating potential drug treatments for SARS-CoV-2. Due to prior knowledge, they know that SARS-CoV-2 leads to the release of cytokines like IL6, which is associated with more severe symptoms and higher mortality in COVID-19 patients \cite{costela-ruiz_sars-cov-2_2020}. They hypothesize that identifying inhibitors of IL6 may provide potential therapeutics for the treatment of SARS-CoV-2. 

They start their investigation by selecting the COVID-19 graph from the available list in the Graphs space. Using their prior knowledge of articles related to cytokine release syndrome in severe COVID-19 cases \cite{zhang_cytokine_2020} and recommended medications for COVID-19 \cite{samaee_tocilizumab_2020, ma_study_2020}, they do a search query using the DOIs of these papers. Highlighted results in the Global View show the causal relationships extracted from these papers (Fig. \ref{fig:teaser}. A). To further examine these results, they click on the ``Open Local View'' button, which displays the corresponding subgraph in the Local View (Fig. \ref{fig:teaser}. B). They then select the IL6 node to open the Drill-down Panel with node metadata  and neighboring relationships. 
They explore the incoming relationships for IL6 and identifies a relationship with SARS-CoV-2, and adds this relationship to the subgraph. They then click on the new relationship to read the underlying evidence, which confirms their prior knowledge i.e. that SARS-CoV-2 increases the amount of IL6.

They continue exploring the subgraph in the Local View and notices that the relationship from tocilizumab to IL6 is encoded in red, which indicates that tocilizumab is an inhibitor of IL-6. They start to wonder if treating a COVID-19 patient with tocilizumab alter their chances of survival.
To better understand the involved biological mechanisms, they click on the edge to read the pieces of evidence underlying this relationship in the Drill-down Panel (Fig. \ref{fig:teaser}. C). In this panel, they see a check-mark beside the relationship heading, indicating that this relationship has been vetted by domain experts and is also supported by 39 pieces of evidence. In this light, they execute a path query that is chained with their prior queries. The results show a pathway from tocilizumab to IL6 to COVID-19, suggesting that tocilizumab (insofar as it acts upon IL6 and therefore could inhibit the cytokine storm) might be a drug candidate for severe COVID-19. Having formulated a hypothesis around tocilizumab and COVID-19 survival rates, they now want to identify if tocilizumab could have any side effects. To explore this, they inspect the 121 outgoing nodes from tocilizumab and see a relationship to immune responses. After adding this relationship to the subgraph, they find that it is of the inhibition type. By inspecting the underlying evidence, they also learn that tocilizumab may lower the ability of the immune system, increasing the risk of superinfections \cite{somers_tocilizumab_2020}. 
Through this quick exploration using our approach, the researcher has been able to quickly identify a potential drug to treat COVID-19 as well as potential side effects. They can continue to expand this line of inquiry to the backing scientific corpus available in the Knowledge space, and look to discover publications and research artifacts related to this drug. They can also choose to explore other biomedical hypotheses across the COVID19 graph, and quickly isolate relevant graph structures and textual support to further analysis.

==> Workshop VIS 2021 - Short paper/sections/7-evaluation.tex <==
\section{Expert Evaluation}

% Domain expert reviews have been shown to generate valuable feedback on visualization tools without the need for a full-fledged user study \cite{tory_evaluating_2005}. 
For an initial assessment on our approach to inform future iteration, we conducted a two-part evaluation: (i) a focus group with five external researchers for high-level feedback; and (ii) an online questionnaire focused on usability and utility with one biomedical researcher with over ten years of experience. All experts conduct research on systems biology, bioinformatics, and causal reasoning using biological models in their daily work.
For the focus group, we presented a demo of the tool before the experts were asked to give general feedback about system function in a group discussion that lasted around two hours. 
For the questionnaire, the expert was first asked to complete a task scenario, which was the same as the usage scenario described in Section \ref{sec:scenario} for investigating potential drug treatments for SARS-CoV-2.
After completing the scenario, the expert was encouraged to keep using the tool, then respond to the questionnaire.

The overall opinion of the domain experts was quite positive regarding the ease of interaction, the scale covered and the overall usefulness of the prototype. %, with comments like \textit{``I found the tool remarkably helpful in navigating the contained knowledge''}. 
Specifically, the experts found the coordination between the Global and Local Views very useful for navigating the contained knowledge. 
%, including comments such as \textit{``I appreciated the Global/Local views, and feel this aids a lot in navigation''}. 
The experts felt that this prototype achieves the goal of supporting query formulation while representing biological relationships in a visually organized way. Some critical feedback received regarded a slight delay when conducting large-scale path queries (due to the query's time-complexity not currently optimized over large graphs), inconsistencies in some path query results (because of path alternatives), and the general need for better notifications. We plan to address all these concerns in the near future. Overall, domain experts agreed that they would like to use the tool frequently as new features, optimizations and improvements continue to be developed. 




==> Workshop VIS 2021 - Short paper/sections/8-conclusions.tex <==
\section{Conclusion and Future Work}

In this paper, we introduced a visual analytics approach for scalable exploration of biomedical knowledge that can aid across a range of biomedical use cases, from disease propagation to drug discovery. To demonstrate the feasibility of our approach, we implemented a web-based prototype that  displays 16 biological models against a corpus of 176,000 documents. Positive feedback from domain experts underscores the usefulness and usability of our prototype in helping them to explore, formulate and validate hypotheses. 

Several promising directions exist in terms of future research. While the Global View is visually scalable for graphs of thousands of nodes and edges, better overviews can be provided to the user via high-level summaries and aggregate graph statistics that surface interactively during graph exploration. Search remains a critical research thread, given the scale and complexity of biological graphs. Highlighting and navigation of search results could be further improved. Search functionality can also better incorporate user context, so more relevant results are returned.
%We will especially work on extending the general capabilities of the prototype by linking the visualization for document clustering and several more components in one single platform. 
% Based on expert feedback, a possible extension would be to allow biomedical researchers to conduct human curation of causal relationships to improve thei were automatically extracted. This would contribute to an overall improvement in the accuracy of the information presented in the Graphs Space. 
Similarly, refinements in the Local View can improve neighborhood suggestions for user-extracted subgraphs. For example, there are almost 2,000 incoming nodes and 1,000 outgoing ones for IL-6 alone in the COVID-19 graph: path ranking based on user context could help prioritize the edge list for the problem at hand. For such global and local improvements, we look to explore graph embedding techniques that convert graph structures into vector representations. Such representations enable various downstream analytic tasks, including similarity search for pathways and subgraphs, path ranking, link prediction and so on. In the Knowledge space, we plan to refine our hierarchical clustering for better visual separation, as well as enrich the view with search capability. We also plan to incorporate citation graphs and add semantic layers such as topics and extracted artifacts to better facilitate exploration across the available corpus.

On the whole, the generality of our approach means it can extend to other workflows that utilize hierarchically organized knowledge graphs that are linked to backing documents. In this way, we believe our approach can be applied to a range of biomedical use-cases and ultimately support knowledge discovery across different scientific domains.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

